RichSpace: Enriching Text-to-Video Prompt Space via Text Embedding Interpolation

Text-to-video generation models have made impressive progress, but they still struggle with generating videos with complex features. This limitation often arises from the inability of the text encoder to produce accurate embeddings, which hinders the video generation model. In this work, we propose a novel approach to overcome this challenge by selecting the optimal text embedding through interpolation in the embedding space. We demonstrate that this method enables the video generation model to produce the desired videos. Additionally, we introduce a simple algorithm using perpendicular foot embeddings and cosine similarity to identify the optimal interpolation embedding. Our findings highlight the importance of accurate text embeddings and offer a pathway for improving text-to-video generation performance.

==> 7_discussion.tex <==
\section{Discussion} \label{sec:discussion}

\paragraph{Identifying the Actual Bottleneck of Generative Models.}
Our work identifies that the primary bottleneck hindering text-to-video generation models from producing the desired videos is the text encoder's inability to generate accurate text embeddings. Through our proposed algorithm, we can guide the video generation model to produce the desired output. This insight helps the community identify the true bottleneck within cutting-edge generative models, allowing for improvements in model performance and capabilities.

\paragraph{Limitations and Future Work.}
As discussed in Section~\ref{sec:experiments}, our algorithm achieves impressive results on various prompts. But there are still some failure cases, which we analyze in Section~\ref{sec:app:failure_cases}. The reason for these failures is that the optimal text embedding may not lie within the linear interpolation space, preventing our algorithm from identifying the correct embedding in such cases. Additionally, leveraging information from $E_{t_c}$ to derive the optimal embedding based on $E_{t_a}$ and $E_{t_b}$ is a non-trivial task. Therefore, we consider this an important direction for future work.
